Flow-Loss: Learning Cardinality Estimates That Matter

Previous approaches to learned cardinality estimation have focused on improving average estimation error, but not all estimates matter equally. Since learned models inevitably make mistakes, the goal should be to improve the estimates that make the biggest difference to an optimizer. We introduce a new loss function, Flow-Loss, that explicitly optimizes for better query plans by approximating the optimizer's cost model and dynamic programming search algorithm with analytical functions. At the heart of Flow-Loss is a reduction of query optimization to a flow routing problem on a certain plan graph in which paths correspond to different query plans. To evaluate our approach, we introduce the Cardinality Estimation Benchmark, which contains the ground truth cardinalities for sub-plans of over 16K queries from 21 templates with up to 15 joins. We show that across different architectures and databases, a model trained with Flow-Loss improves the cost of plans (using the PostgreSQL cost model) and query runtimes despite having worse estimation accuracy than a model trained with Q-Error. When the test set queries closely match the training queries, both models improve performance significantly over PostgreSQL and are close to the optimal performance (using true cardinalities). However, the Q-Error trained model degrades significantly when evaluated on queries that are slightly different (e.g., similar but not identical query templates), while the Flow-Loss trained model generalizes better to such situations. For example, the Flow-Loss model achieves up to 1.5x better runtimes on unseen templates compared to the Q-Error model, despite leveraging the same model architecture and training data.

==> experiments.tex <==



\section{Experiments}

\vspace{2mm} \noindent Evaluation Metrics

Our focus is to understand how \FlowLoss compares to other loss functions while keeping the model architecture the same. We will consider two scenarios. In the first scenario, we will evaluate how well a model does when the queries are similar to the ones it was trained on. In the second scenario, we evaluate how robust are these models when the queries diverge from the training distribution. In a sense, the second scenario tests how badly can things go wrong when there are slight shifts in the workload. 

\subsection{Experiment 1}

We train each model on $50\%$ of queries for each of the $15$ \CEB templates. This corresponds to $6819$ queries, and around $1.6$ million sub-queries. We will evaluate them on two workloads

\begin{enumerate}
    \item In Distribution Dataset: This consists of the remaining $50\%$ unseen queries in \CEB.
    \item Out-of Distribution Dataset: This consists of the $113$ queries from JOB. The JOB queries are on the same IMDb database, but include tables and columns that are not seen in \CEB. Since we assume a featurization that is consistent for the whole database schema, this means that there will be spots in the feature vector which were never seen in the training data, but there is also a large overlap of query sub-graphs that are common to both \CEB and JOB. 
\end{enumerate}


Figure \ref{fig:res-all} captures the essence of our results. We show the mean \PostgresError and Runtimes for the MSCN model trained using Q-Error, Q-Error with Priority or \FlowLoss. For the In-Distribution case, we see that the model trained on \FlowLoss is clearly better in terms of \PostgresError, as we had hoped to achieve. This improvement does not quite translate into significant runtime improvements. Partially, this is because the PostgreSQL cost model is only an approximation for the runtimes. But also, a lot of these $6800$ queries run extremely fast - even under $1$ second - so we need to look at the tails to see a difference in performance. More crucial is how the performance of the Q-Error trained models degrade when we switch the workload. These models share the same architecture and perform reasonably in the usual, in-distribution scenario. So it was definitely possible to learn a model that adapts better to the changes in the JOB workload. But only the \FlowLoss trained model appears to learn features which generalize well. Let us now dive deeper into the results by looking beyond the mean values.

\vspace{2mm} \noindent \textbf{MSCN Q-Error, MSCN Priority, and MSCN \FlowLoss: In Distribution} To dive deeper into the In-Distribution results, let us look at Tables \ref{tab:all-test}, which presents the distributions of all three error metrics: Q-Error, \PostgresError, and Runtimes along with other baselines. The fixed baselines, True and Postgres, evaluate these metrics with true cardinalities and the PostgreSQL estimates respectively. We can think of True as a lower bound on the runtimes since the cost model, and optimizer are the same, so cardinality errors can lead to faster runtimes only in accidental cases. Similarly, Postgres can be considered an upper bound in the In-Distribution scenario, as these estimates are provided as features for each of these models - so it is easy to improve upon them. The MSCN Q-Error and MSCN Priority models do clearly better than \FlowLoss on Q-Error. This is not surprising, as both optimize for Q-Error while training. But our goal was to improve on \PostgresError, and \FlowLoss does significantly better here: almost $10x$ better in the $90th$ percentile, and $5x$ in the $99th$ percentile. This strongly suggests that optimizing for \FlowLoss may be closer to the process of query optimization. The \FlowLoss trained model closely tracks the True runtimes right up to the $99th$ percentile - while we can see the gap with the other MSCN models increase. In this sense, the \FlowLoss model does as well as one could hope for. 

\vspace{2mm} \noindent \textbf{MSCN Q-Error, MSCN Priority, and MSCN \FlowLoss: Out of Distribution} Since many of the query sub-graphs on the JOB workload were not present in the \CEB queries, it is not surprising that all models have some extremely bad cardinality estimates. But the MSCN \FlowLoss model does clearly better in terms of Q-Error, being under $10$ in the median. More crucially, both the MSCN Q-Error, and MSCN Priority models have large regressions on \PostgresError compared to the default Postgres estimates, despite having the cardinality estimates from Postgres as input features. In contrast, the \FlowLoss trained model clearly improves on the Postgres baseline, again being extremely close to optimal both in terms of \PostgresError and Runtimes.

\vspace{2mm} \noindent \textbf{Alternative Featurization with Sample Bitmaps}

Under the MSCN w/ Sample Bitmaps section of Tables \ref{tab:all-test} and \ref{tab:all-job}, we present the same experiments with the sample bitmaps featurization. Sample bitmaps provide much more information about the base table predicates - but this comes at a cost: the model size is $4x$ larger (Figure \ref{fig:model_sizes}), and the size of the input feature vectors for each query increases from $1400$ to $6400$. Qualitatively, our key takeaway is the same: all the models perform similarly on \CEB, but only the \FlowLoss trained model generalizes to JOB - being almost $10x-20x$ better on \PostgresError, and having these improvements reflect in the Runtimes as well. 

The additional features help both the Q-Error based models improve their performance on the In-Distribution queries. Counter intuitively, the additional features lead to a slightly worse performance for the \FlowLoss model. This appears to be due to the inconsistencies between our simple cost model, $\phi$, and PostgreSQL's cost model. In particular, the \FlowLoss trained model seems to be able to use the additional features provided by the sample bitmaps to do well on on \FlowLoss while having higher Q-Error than in our main featurization scheme. But size thresholds are more important in PostgreSQL's cost model, and it leads to worse outliers on \PostgresError - compared to the \FlowLoss model without sample bitmaps, it is only worse in the $99th$ percentile. But as we see in various experiments, a few $100k$ units on the PostgreSQL cost model does not seem to translate to significant changes in the runtimes. Thus, we believe the generalization behavior is more crucial.


\input{fig_tex_files/exp1_all_results_table.tex}
\input{fig_tex_files/exp1_all_results_job.tex}
\input{fig_tex_files/exp1_stackexchange_all_table}




Typically simpler models generalize better, but at the cost of sacrificing performance when the evaluation set closely matches the training set. But the model trained on \FlowLoss was close to optimal in the In-Distribution scenario, while generalizing better to JOB. We hypothesize that the improved robustness to new types of queries was because it does not spend model capacity to fit noisy cardinality estimates that are not as important for the quality of query plans. This can let it learn to use features that are more robust, such as the Postgres estimates, which have more meaningful value in the out of distribution settings. But JOB is a significantly smaller, and less challenging workload than \CEB - for instance, the Postgres baseline does $10x$ worse on \CEB than on JOB, as can be seen from Tables \ref{tab:all-job} and \ref{tab:all-test}. To validate our hypothesis, we designed a more challenging experiment to test for generalization.



\input{fig_tex_files/so_results_diff}


==> fig_tex_files/exp1_all_results_job.tex <==
\begin{table*}
\centering

\begin{tabular}{l|llll|llll|llll}
&
\multicolumn{4}{c}{\textbf{Q-Error}} &  \multicolumn{4}{c}{\textbf{\PostgresError}} &  \multicolumn{4}{c}{\textbf{Runtimes}} &

\textbf{Estimator} & Mean & 50P & 90P & 99P & Mean & 50P & 90P & 99P & Mean & 50P & 90P & 99P  \\  

\hline
\multicolumn{2}{l}{\textbf{Fixed Baselines}} & &   \\
True &        1.00 &    1.00 &       1.00 &         1.00  &        0.00 &       0 &        0 &  0 &  14.80 &   4.56 &  25.96 &  240.39     \\ 
Postgres &    73K &  260 &   42K &   1.4M &   472K &   36K &   800K &  6.5M &  18.78 &   5.65 &  38.82 &  252.39  \\ 



\multicolumn{2}{l}{\textbf{MVCN}} & \\

MVCN Q-Error &  3M &  238 &  156K &  14M &  5.2M &   48K &  2.6M &  9.5M &  54.04 &   7.54 &  57.01 &  860.17  \\ 
MVCN Priority & 19M &  204.35 &  253K &  64M &  865K &  66K & 1.9M &  10M & 18.74 &  6.06 & 37.84 & 248.36 \\
MVCN - \FlowLoss & 910 &    9.47 &     588 &    14K & 168K &   2K &   290K &   2M &  15.54 &   4.73 &  31.67 &  223.72    \\ 

\multicolumn{2}{l}{\textbf{Sample Bitmap Features}} & \\


\end{tabular}
\caption{Out-of-Distribution Test Set (JOB)}
\label{tab:all-job}
\end{table*}



==> fig_tex_files/exp1_all_results_table.tex <==
\begin{table*}
\centering

\begin{tabular}{l|llll|llll|llll}
&
\multicolumn{4}{c}{\textbf{Q-Error}} &  \multicolumn{4}{c}{\textbf{\PostgresError}} &  \multicolumn{4}{c}{\textbf{Runtimes}} &

\textbf{Estimator} & Mean & 50P & 90P & 99P & Mean & 50P & 90P & 99P & Mean & 50P & 90P & 99P  \\  

\hline
\multicolumn{2}{l}{\textbf{Fixed Baselines}} & &   \\

True &        1.00 &    1.00 &       1.00 &         1.00  & 0 & 0 & 0 & 0  &  13.23 &   9.17 &  28.96 &   60.83 \\ 
Postgres &   134K &   42.87 &   48K &   2.2M  &  6.048M &  417K &  6.86M &  94M &  20.86 &  14.11 &  46.86 &  101.57  \\


\multicolumn{2}{l}{\textbf{FCNN}} & \\


FCNN - Q-Error & 12.09 &  1.95 &    8.71 &   100.74 & 1.48M &  6K & 501K & 10M & 13.83 & 9.62 & 30.82 &  60.10  \\ 
FCNN - \Priority & 16.94 &  2.02 &    9.57 &   128.60 & 604K &  5K & 412K &  5M   \\

FCNN - \FlowLoss &  72.99 &  3.07 &   28.01 &   807.53 &  815K & 25K & 767K &  5.9M & 13.93 & 9.72 & 30.97 &  60.50   \\ 

\multicolumn{2}{l}{\textbf{MSCN}} & \\

MSCN - Q-Error &  13.34 &  2.00 &    9.53 &   101.77 & 1.88M & 12K & 610K & 12M & 13.69 & 9.51 & 30.49 &  58.49  \\ 

MSCN - \Priority & 14.81 &  2.34 &   12.83 &   146.90 & 987K & 12K & 586K &  8.4M & 13.83 & 9.45 & 31.10 &  60.00 \\

MSCN - \FlowLoss & 186.21 &  2.94 &   42.90 &  2065.14 & 1.04M & 41K & 903K & 11M & 14.08 & 9.97 & 31.61 &  59.88    \\ 


\multicolumn{2}{l}{\textbf{Sample Bitmap Features}} & \\




\end{tabular}
\caption{Models trained on the same IMDb templates}
\label{tab:imdb-all-test}
\end{table*}



==> fig_tex_files/exp1_stackexchange_all_table.tex <==
\begin{table*}
\centering

\begin{tabular}{l|lll|llll|llll}
&
\multicolumn{3}{c}{\textbf{Q-Error}} &  \multicolumn{4}{c}{\textbf{\PostgresError}} &  \multicolumn{4}{c}{\textbf{Runtimes}} &

\textbf{Estimator} & 50P & 90P & 99P & Mean & 50P & 90P & 99P & Mean & 50P & 90P & 99P  \\  

\hline
\multicolumn{2}{l}{\textbf{Fixed Baselines}} & &   \\

True &     1.00 &    1.00 &      1.00  & 0 & 0 & 0 & 0 & 26.76 & 13.94 &  72.29 & 126.85  \\ 
Postgres &   1.14 & 1444.12 & 1763K &  92.6M & 1.12M & 212M & 1.3B & 76.37 & 13.49 & 133.03 & 909.00  \\


\multicolumn{2}{l}{\textbf{FCNN}} & \\

FCNN Q-Error &    1.3 $\pm$ 0.05 &   51 $\pm$ 41 & 2.7K $\pm$ 1.4K  & 20M $\pm$ 17M &  16K $\pm$ 3K &   600K $\pm$ 70K &  5.8M $\pm$ 1M & 35.91 & 20.58 &  89.47 & 139.79     \\ 

FCNN - \FlowLoss &  20 $\pm$ 4 &  325 $\pm$ 47 &   5K $\pm$ 1K & 15M $\pm$ 10M &  50K $\pm$ 3K &   6M $\pm$ 50K & 37M $\pm$ 2M & 31.57 & 12.94 & 90.09 & 153.93    \\ 

\multicolumn{2}{l}{\textbf{MSCN}} & \\

MSCN Q-Error &    1.83 $\pm$ 0.46 &   15 $\pm$ 4 & 100 $\pm$ 0  & 4.8M $\pm$ 10M &  52K $\pm$ 11K &   790K $\pm$ 77K &  5M $\pm$ 1M & 29.65 &  9.56 & 84.36 & 159.84      \\ 

MSCN - \FlowLoss &  18 $\pm$ 5 &  683 $\pm$ 276 &   9K $\pm$ 3K & 6.3M $\pm$ 8M &  180K $\pm$ 79K &   4M $\pm$ 1M & 34M $\pm$ 2M & 34.51 & 23.97 & 87.26 & 122.02   \\ 

\end{tabular}
\centering
\caption{Models trained on same StackExchange templates (different queries)}
\label{tab:all-test}
\end{table*}

==> fig_tex_files/exp_diff_rts.tex <==
\begin{figure}[hbtp]
    \centering
    \begin{subfigure}[b]{0.47\textwidth}
        \centering
        \includegraphics[width=\textwidth]{exp_diff_imgs/Runtimes-test-Box-{'postgres', 'mse', 'flow_loss2', 'mse_priority'}.png}

        \label{fig:exp_diff_rts}
    \end{subfigure}%
    \caption[]%
    {{\small Runtimes across the first seven training - test templates splits, based on random seeds 1-7. The timeout was set at $900$ seconds, and are shown as reaching the top of the y-axis in the figure.}}    
\end{figure}

==> fig_tex_files/so_results_diff.tex <==
\begin{figure*}[hbtp]
    \centering
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=\textwidth]{exp_diff_imgs/so-mscn-fcnn-testdiff.png}
        \caption[]%
        {{\small QError}}    
        \label{fig:exp1_qerr1}
    \end{subfigure}
    \label{fig:res_diff_summary}
    \caption{Summary: Experiment with unseen templates in Test Set, with 50 different splits}
\end{figure*}

==> intro.tex <==
\section{Introduction}

\begin{figure}[t]
  \begin{minipage}[b]{1.0 \linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{intro_imgs/example.png}
    \caption{With true cardinality values, the query optimizer will choose Plan1 over Plan2 due to its smaller cost. This is also the case with Estimator1. Interestingly, although Estimator2’s cardinality values have smaller error than those of Estimator1, they will mislead the optimizer to choose Plan2.}
    \vspace{8ex}
    \label{fig:eg1}
  \end{minipage}%
\end{figure}

Previous work has shown that reasonably accurate cardinality estimates for intermediate result sizes are key to the query optimizer to choose between alternative query plans. %
However, not all estimates are equally important.
While the optimizer may be very sensitive to certain estimates, it may not be affected by others at all.

Meanwhile, recent approaches to cardinality estimation based on machine learning have shown success in improving estimation accuracy. %
While these works use query optimization as their main motivation for improved estimates, they largely neglect the impact of these estimates on query plans and runtimes.
Hence, the question arises whether the accuracy gains achieved by these recent proposals actually make a difference in practice.
A study by Ortiz et al. shows that the improved estimation accuracy by learned models can positively impact query plans. %
While this study is a step into the right direction, we argue that there is a lot of untapped potential w.r.t. impact on query performance due to the decoupling of cardinality estimation and query optimization in existing approaches.

For instance, consider the example in Figure \ref{fig:eg1}: improving the cardinality estimate of just one join ($A \Join C$) actually leads to the optimizer finding a worse plan (Plan B), because the relative cardinalities are not quite right.
And this is not an isolated example: all cardinality estimators will have non-trivial error components due to bounds on the model complexity, size, and inference time.
By focusing on the downstream task, of query optimization, we seek to focus the limited capacity of models on areas which will be most impacted by more precise cardinality estimates. A few intuitive examples are:

\begin{enumerate}
    \item In many cases, it may be enough for the optimizer to just be able to say that A would be much larger or much smaller than B. Here, it is crucial to note that the relative sizes of alternative join paths are very important, but it is not easy to encode this, and learn cardinalities based on it.
    \item For joins that are seen often, especially, with fewer tables, we may need much more precise estimates than for joins with many more tables. But these heuristics do not apply uniformly to all situations, and it is easy to construct counterexamples where they will not hold.
\end{enumerate}

Another drawback of some current learned cardinality modules is that they focus on single-table selectivity estimates and do not support joins.
While improved selectivity estimates may be important in other contexts, such as approximate query processing (AQP), we believe that single-table estimates are a solved problem in the context of query optimization.
With (materialized) samples one can get a reasonably good estimate on the selectivity of a selection.
While sampling has its issues in low selectivity cases, we argue that the absolute estimates in such cases are not important for the optimizer.
That is, if none of 1,000 sample tuples qualifies a selection, we know that its selectivity is likely below 0.1\% which will be a good enough estimate for the optimizer.
Using join sampling to extend single-table models to joins is arguably a non-straightforward endeavour. %

Part of the reason why many proposals do not study the impact on query plans (which notably include joins) is the lack of a standard benchmark.
While the Join Order Benchmark (JOB) addresses this problem by covering edge cases and complex expressions (e.g., LIKE) which are difficult for optimizers, it only contains a limited number of queries.
As one of our contributions, we propose an extensive benchmark on the Internet Movie Database (IMDb) schema.

With this work, we address the aforementioned drawbacks of learned cardinality estimation.
Our overarching goal is to learn a cardinality estimation model with the objective to improve query performance.
We are not after a heuristic that models certain cases, but would like to have a loss function that implicitly puts more emphasis on the estimates that make a difference to a given query workload.
As a replacement for the well-known Q-Error loss function used by existing approaches, we propose \FlowLoss, a loss function that also accounts for the impact of cardinality estimates.
At its core, our technique involves computing the gradient of the cost of a query plan with respect to the cardinality estimates.
This lets us use gradient descent-based techniques to improve the cardinality estimates that are most relevant to improving the plan of a given query.
To do this, we assume a simplified cost model and model the dynamic program algorithm for query optimization on left deep plans as a shortest path problem.
Then, we approximate this with a smooth and differentiable objective which is easy to optimize for.
We show that improving cardinalities with respect to this objective also improves the quality of plans of the complex PostgreSQL optimizer.

Intuitively, \FlowLoss finds which parts of a query are more important from the perspective of query optimization.
Then, a supervised learning model can focus its limited capacity on robustly estimating these higher priority queries, without overfitting to the rest of the noisy training data, similar to how transformer and attention-based models in natural language processing lead to significant improvements by treating certain input sections as more important than others \cite{transformer1, transformer2}.


Our key contributions are:
\begin{itemize}
    \item We revisit Plan-Cost originally defined by Moerkotte et al.~\cite{neumann_qerror}, which measures the impact of cardinality estimation errors on the quality of plans produced by the optimizer. We show that this metric correlates closely with runtimes, thus it is a more suitable metric to evaluate estimation errors when our goal is query optimization.
    \item We introduce \FlowLoss, which is a smooth and differentiable approximation of Plan Error, that can be optimized by any supervised learning model with gradient descent. It also gives us a way to quantify which parts of a query are more important than others, which can have other uses, such as when training unsupervised cardinality estimation models.
    \item We create a new tool that can be used to generate a large amount of challenging queries based on templates in a semi-automated way. We introduce a new benchmark, \OurDataset, created using this tool. This benchmark is over $100x$ larger than the Join Order Benchmark, but has similarly challenging queries.
    \item Collecting ground truth data is an expensive process, especially for larger queries. We show that we can achieve similar model performance by training on data collected using approximate query processing techniques, while taking $10-100x$ less time than collecting ground truth data.
\end{itemize}




\input{fig_tex_files/flow_loss_overview2.tex}

==> prioritized_qerror.tex <==
\section{Prioritized Q-Error \label{sec:pr_qerror}}

As an alternative to \FlowLoss, we propose another training method that seeks to indirectly get the same benefits.



==> sysmod.tex <==
\section{System model}
\label{sec:sysmod}
